Top Pass: Improve Code Generation by Pass@k-Maximized Code Ranking

Code generation has been greatly enhanced by the profound advancements in Large Language Models (LLMs) recently. Nevertheless, such LLM-based code generation approaches still struggle to generate error-free code in a few tries when faced with complex problems. To address this, the prevailing strategy is to sample a huge number of candidate programs, with the hope of any one in them could work. However, users of code generation systems usually expect to find a correct program by reviewing or testing only a small number of code candidates. Otherwise, the system would be unhelpful. In this paper, we propose Top Pass, a code ranking approach that identifies potential correct solutions from a large number of candidates. Top Pass directly optimizes the pass@k loss function, enhancing the quality at the top of the candidate list. This enables the user to find the correct solution within as few tries as possible. Experimental results on four benchmarks indicate that our Top Pass method enhances the usability of code generation models by producing better ranking results, particularly achieving a 32.9\% relative improvement in pass@1 on CodeContests when compared to the state-of-the-art ranking method.

==> tables/hyperparameter_pq.tex <==
\setcellformat[l]{00.0}{}{000.0}

\centering
\small
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllll}
\toprule
\textbf{p} & \textbf{q} & \textbf{Pass@1} &  \textbf{Pass@2} & \textbf{Pass@3} & \textbf{Pass@5} & \textbf{Pass@10}\\
\midrule
0.6 & 0.4 & \msc{7.9} & \msc{13.9} & \msc{15.2} & \msc{15.8} & \msc{18.2}   \\
0.7 & 0.4 & \msc{7.9} & \msc{12.1} & \msc{13.3} & \msc{16.4} & \msc{19.4}   \\
0.8 & 0.4 & \msc{7.9} & \msc{8.5} & \msc{11.5} & \msc{16.4} & \msc{17.0}   \\
0.9 & 0.4 & \msc{8.5} & \msc{10.3} & \msc{12.7} & \msc{15.8} & \msc{17.6}   \\
1.0 & 0.4 & \msc{7.9} & \msc{9.7}  & \msc{10.3} & \msc{13.9}  & \msc{17.6}    \\
\midrule
0.6 & 0.5 & \msc{7.3} & \msc{12.7} & \msc{15.2} & \msc{15.8} & \msc{17.6}   \\
0.7 & 0.5 & \msc{7.9} & \msc{10.9} & \msc{12.1} & \msc{13.9} & \msc{17.6}   \\
0.8 & 0.5 & \msc{8.5} & \msc{10.3} & \msc{12.7} & \msc{16.4} & \msc{19.4}   \\
0.9 & 0.5 & \msc{9.7} & \msc{12.7} & \msc{13.3} & \msc{14.5} & \msc{18.2}   \\
1.0 & 0.5 & \msc{8.5} & \msc{9.1}  & \msc{10.3} & \msc{12.1}  & \msc{13.9}    \\
\midrule
0.6 & 0.6 & \msc{7.3} & \msc{9.7} & \msc{11.5} & \msc{13.3} & \msc{15.8}   \\
0.7 & 0.6 & \msc{7.3} & \msc{8.5} & \msc{12.1} & \msc{15.8} & \msc{17.6}   \\
0.8 & 0.6 & \msc{7.3} & \msc{9.1} & \msc{10.9} & \msc{12.7} & \msc{16.4}   \\
0.9 & 0.6 & \msc{8.5} & \msc{10.3} & \msc{12.1} & \msc{15.2} & \msc{17.0}   \\
1.0 & 0.6 & \msc{7.9} & \msc{9.1}  & \msc{10.3} & \msc{11.5}  & \msc{17.0}    \\
\midrule
0.6 & 0.7 & \msc{7.3} & \msc{10.9} & \msc{12.1} & \msc{15.2} & \msc{17.0}   \\
0.7 & 0.7 & \msc{7.3} & \msc{10.9} & \msc{12.1} & \msc{12.7} & \msc{17.0}   \\
0.8 & 0.7 & \msc{7.9} & \msc{9.1} & \msc{10.9} & \msc{14.5} & \msc{19.4}   \\
0.9 & 0.7 & \msc{7.9} & \msc{9.1} & \msc{10.9} & \msc{13.3} & \msc{16.4}   \\
1.0 & 0.7 & \msc{7.9} &\msc{9.1}  & \msc{10.3} & \msc{13.9}  & \msc{17.0}    \\


\bottomrule
\end{tabular}
}


==> tables/tabcmd_text.tex <==
% Cell alignment command for mean +/- std (text version).
% 
% Author: Zheng Xie
% Date: 2024.01.07
% 
% This file provides an alternative (and sometimes better) way for producing 
% aligned column of mean +/- std, than using siunitx package.
% 
% By calling:
%     \msc{90.12}         (for mean only), or 
%     \msc{90.12,}        (for mean only, but align with cells with std's), or 
%     \msc{90.12,3.45}    (for mean +/- std),
% the column will be aligned at the separator, the decimal point of the mean (if
% all means have the same digits after decimal point), and the decimal point of 
% the std (if all std's have the same digits before decimal point). The overall 
% column can be aligned left/right/centered according to the tabular options. 
% The numbers will be in math font, the std will be printed as subscripts.
% To bold the cell, just call:
%     \msc[b]{90.12,3.45} 
% or simply
%     \msb{90.12,3.45}   
% A key advantage of this command is that the bold font is implemented to be of 
% the same width of normal numbers, so that making cells bold does not affect
% alignment.
% 
% You can use the command:
%     \setcellformat[std alignment]{mean format}{sep}{std format}
% at the beginning of the table to setup the command.
% example:
%     \setcellformat[l/r]{00.00}{\ensuremath{_\pm}}{00.00}
% the default setting is:
%     \setcellformat[l]{00.00}{\ensuremath{_\pm}}{00.00}
% If you want to use the mean only, its recommended to set the last two options
% empty so that the numbers are not shifted to the left.
% 
% The mean/std format determines the space the number will taken. Making std 
% align to the left is the default option, which usually make the numbers close 
% to the separator but not aligned at their decimal points if they have 
% different magnitudes. 
% 
% Other examples:
% Highlighting the percentage of increment:
%     \renewcommand{\basicstdstyle}[1]{{\color{red} +#1\%}}
%     \setcellformat[l]{00.00}{}{00.00}
% Put the std in parentheses:
%     \renewcommand{\basicstdstyle}[1]{(#1)}
%     \setcellformat[l]{00.00}{}{00.00}

\newcommand\msmfmt{00.00}
\newcommand\mssep{\ensuremath{_\pm}}
\newcommand\mssfmt{\textsubscript{00.00}}
\newcommand\msstdalign{l}

\newcommand{\basicmeanstyle}[1]{#1}%
\newcommand{\basicstdstyle}[1]{#1}%
\newcommand*\bfmeanstyle[1]{\textbf{\basicmeanstyle{#1}}}%
\newcommand*\bfstdstyle[1]{\textbf{\basicstdstyle{#1}}}%

\newlength{\meanlen}
\newlength{\stdlen}
\settowidth{\meanlen}{{\basicmeanstyle{\msmfmt}}}
\settowidth{\stdlen}{{\basicstdstyle{\mssfmt}}}

\newcommand{\meanstyle}[1]{\basicstdstyle{#1}}%
\newcommand{\stdstyle}[1]{\basicstdstyle{#1}}%

\newcommand{\msprintmean}[1]{{\makebox[\meanlen][r]{\meanstyle{#1}}}}
\newcommand{\msprintstd}[1]{\mssep{\makebox[\stdlen][\msstdalign]{\textsubscript{\stdstyle{#1}}}}}

\newcommand{\setcellformat}[4][l]{
    \renewcommand\msstdalign{#1}%
    \renewcommand\msmfmt{#2}%
    \renewcommand\mssep{#3}%
    \renewcommand\mssfmt{\textsubscript{#4}}%
    \settowidth{\meanlen}{{\msmfmt}}%
    \settowidth{\stdlen}{{\mssfmt}}%
}
% default: \setcellformat[l]{00.00}{\ensuremath{\pm}}{00.00}



\newcommand{\msc}[2][n]{%
    \let\meanstyle\basicmeanstyle%
    \let\stdstyle\basicstdstyle%
    \ifx b#1\let\meanstyle\bfmeanstyle\let\stdstyle\bfstdstyle\fi%
	\setsepchar{,}%
    \reademptyitems%
	\readlist*\theparam{#2}%
    \ignoreemptyitems%
	\readlist*\theneparam{#2}%
    \msprintmean{\theparam[1]}%
    \ifnum \theparamlen=2 
        \ifnum \theneparamlen=2
            \msprintstd{\theparam[2]}%
        \else
            \phantom{\msprintstd{0}}%
        \fi
    \fi
}

\newcommand{\msb}[1]{\msc[b]{#1}}


